DEUS: Distributed Electronic Patient File Update System

Inadequate availability of patient information is a major cause for medical errors and affects costs in healthcare. Traditional approaches to information integration in healthcare do not solve the problem. Applying a document-oriented paradigm to systems integration enables inter-institutional information exchange in healthcare. The goal of the proposed architecture is to provide information exchange between strict autonomous healthcare institutions, bridging the gap between primary and secondary care. In a long-term healthcare data distribution scenario, the patient has to maintain sovereignty over any personal health information. Thus, the traditional publish-subscribe architecture is extended by a phase of human mediation within the data flow. DEUS essentially decouples the roles of information author and information publisher into distinct actors, resulting in a triangular data flow. The interaction scenario will be motivated. The significance of human mediation will be discussed. DEUS provides a carefully distinguished actor and role model for mediated pub-sub. The data flow between the participants is factored into distinct phases of information interchange. The artefact model is decomposed into role-dependent constituent parts. Both a domain specific (healthcare) terminology and a generic terminology is provided. From a technical perspective, the system design is presented. The sublayer for network transfer will be highlighted as well as the subsystem for human-machine interaction.

==> 02_authors_truth.tex <==
%auto-ignore
% You need the command \numberofauthors to handle the 'placement
% and alignment' of the authors beneath the title.
%
% For aesthetic reasons, we recommend 'three authors at a time'
% i.e. three 'name/affiliation blocks' be placed beneath the title.
%
% NOTE: You are NOT restricted in how many 'rows' of
% "name/affiliations" may appear. We just ask that you restrict
% the number of 'columns' to three.
%
% Because of the available 'opening page real-estate'
% we ask you to refrain from putting more than six authors
% (two rows with three columns) beneath the article title.
% More than six makes the first-page appear very cluttered indeed.
%
% Use the \alignauthor commands to handle the names
% and affiliations for an 'aesthetic maximum' of six authors.
% Add names, affiliations, addresses for
% the seventh etc. author(s) as the argument for the
% \additionalauthors command.
% These 'additional authors' will be output/set for you
% without further effort on your part as the last section in
% the body of your article BEFORE References or any Appendices.
\numberofauthors{4} %  in this sample file, there are a *total*
% of EIGHT authors. SIX appear on the 'first-page' (for formatting
% reasons) and the remaining two appear in the \additionalauthors section.
%
%%% AUTHORS:BEGIN
\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
\alignauthor
Christoph P.\,Neumann\\
%       \affaddr{Department of Computer Science}\\
%       \affaddr{Martensstr. 3}\\
%       \affaddr{Erlangen, Germany}\\
       \email{cpn@i6.cs.fau.de}
% 2nd. author
\alignauthor
Florian Rampp\\
%       \affaddr{Department of Computer Science}\\
%       \affaddr{Martensstr. 3}\\
%       \affaddr{Erlangen, Germany}\\
       \email{siflramp@i6.cs.fau.de}
% 3rd. author
\alignauthor
Michael Daum\\
%       \affaddr{Department of Computer Science}\\
%       \affaddr{Martensstr. 3}\\
%       \affaddr{Erlangen, Germany}\\
       \email{md@i6.cs.fau.de}
\and
\alignauthor
% 4th. author
\alignauthor
Richard Lenz\\
%       \affaddr{Department of Computer Science}\\
%       \affaddr{Martensstr. 3}\\
%       \affaddr{Erlangen, Germany}\\
       \email{rl@cs.fau.de}
%     
\alignauthor
%
%%% SHARED AFFILITION
\sharedaffiliation
%
      \affaddr{Institute of Computer Science 6 (Data Management)}\\
      \affaddr{University of Erlangen-Nuremberg}\\
      \affaddr{Erlangen, Germany}
%%% AUTHORS:END
}
